Lossless Compression with Probabilistic Circuits

Despite extensive progress on image generation, common deep generative model architectures are not easily applied to lossless compression. For example, VAEs suffer from a compression cost overhead due to their latent variables. This overhead can only be partially eliminated with elaborate schemes such as bits-back coding, often resulting in poor single-sample compression rates. To overcome such problems, we establish a new class of tractable lossless compression models that permit efficient encoding and decoding: Probabilistic Circuits (PCs). These are a class of neural networks involving $|p|$ computational units that support efficient marginalization over arbitrary subsets of the $D$ feature dimensions, enabling efficient arithmetic coding. We derive efficient encoding and decoding schemes that both have time complexity $\mathcal{O} (\log(D) \cdot |p|)$, where a naive scheme would have linear costs in $D$ and $|p|$, making the approach highly scalable. Empirically, our PC-based (de)compression algorithm runs 5-40 times faster than neural compression algorithms that achieve similar bitrates. By scaling up the traditional PC structure learning pipeline, we achieve state-of-the-art results on image datasets such as MNIST. Furthermore, PCs can be naturally integrated with existing neural compression algorithms to improve the performance of these base models on natural image datasets. Our results highlight the potential impact that non-standard learning architectures may have on neural data compression.

==> archived.tex <==
\begin{figure}[t]
\begin{minipage}[t]{0.49\textwidth}

\begin{algorithm}[H]
\caption{Compress}
\label{alg:compress}
{\fontsize{9}{9} \selectfont
\begin{algorithmic}[1]

\STATE {\bfseries Input:} A smooth and SD PC $\p$ and sample $\x$

\STATE {\bfseries Output:} Bitstring $b$

\STATE {\bfseries Require:} rANS \citep{duda2013asymmetric}

\STATE $\pi^{*} \!\leftarrow\! \text{optimal~variable~order~of~} \p$ (see \cref{sec:proof-sd-pc}) \vspace{0.2em}

\FOR{\tikzmarknode{a1}{} $i = 1 \text{~\textbf{to}~} K$}

\STATE Compute $r_{l,i} (\x)$ and $r_{h,i} (\x)$ (\cref{eq:dec-ranges-1,eq:dec-ranges-2})

\ENDFOR

\STATE Initialize bitstring $b$ used by rANS

\FOR{\tikzmarknode{a2}{} $i = K \text{~\textbf{to}~} 1$}

\STATE Encode $[r_{l,i} (\x), r_{h,i} (\x))$ into $b$ using rANS

\ENDFOR

\STATE {\bfseries return} $b$

\end{algorithmic}
}
\end{algorithm}

\end{minipage}
\begin{minipage}[t]{0.5\textwidth}

\begin{algorithm}[H]
\caption{Decompress}
\label{alg:decompress}
{\fontsize{9}{9} \selectfont
\begin{algorithmic}[1]

\STATE {\bfseries Input:} A smooth and SD PC $\p$ and bitstring $b$

\STATE {\bfseries Output:} Sample $\x$

\STATE {\bfseries Require:} rANS \vspace{0.1em}

\NoDo
\FOR{\tikzmarknode{b1}{} $i = 1 \text{~\textbf{to}~} K$ \textbf{do} $\#$ Decode the value of $X_{\pi^{*}_{i}}$}

\STATE \vspace{-0.2em} $z \leftarrow \text{number~decoded~from~} b \text{~with~rANS}$

\STATE{Use binary search to find $x_{\pi^{*}_{i}}$ such that 
    {\setlength{\abovedisplayskip}{0.0em}
    \setlength{\belowdisplayskip}{-0.7em}
    \begin{align*}
        r_{l,i} (\x) \leq z < r_{h,i} (\x)
    \end{align*}}
}

\STATE Update $b$ with $f(x_{\pi^{*}_{i}})$ and $g(x_{\pi^{*}_{i}})$ using rANS

\ENDFOR
\ReDo

\STATE {\bfseries return} $\x := \{x_{\pi^{*}_{i}}\}_{i=1}^{K}$ \vspace{-0.2em}

\end{algorithmic}
}
\end{algorithm}

\end{minipage}
\begin{tikzpicture}[overlay,remember picture]
    \draw[black,line width=0.6pt] ([xshift=-10pt,yshift=-3pt]a1.west) -- ([xshift=-10pt,yshift=-24pt]a1.west) -- ([xshift=-6pt,yshift=-24pt]a1.west);
    \draw[black,line width=0.6pt] ([xshift=-10pt,yshift=-3pt]a2.west) -- ([xshift=-10pt,yshift=-10pt]a2.west) -- ([xshift=-6pt,yshift=-10pt]a2.west);
    \draw[black,line width=0.6pt] ([xshift=-10pt,yshift=-3pt]b1.west) -- ([xshift=-10pt,yshift=-60pt]b1.west) -- ([xshift=-6pt,yshift=-60pt]b1.west);
\end{tikzpicture}
\vspace{-1.4em}
\end{figure}

% Assume we have learned expressive PC models, our next goal is to develop compression and decompression algorithms that are both \emph{optimal} (in the sense that it can achieve practical compression rates close to the lower-bound specified by Shannon's source coding theorem) and \emph{computationally efficient}. In the following, we take gradual steps to introduce the theoretically-grounded (de)compression algorithms for PC that are both fast and near optimal. Specifically, \cref{sec:background-compression} introduces relevant background on lossless compression; \cref{sec:rANS} provides a high-level sketch of the algorithms, highlighting the importance of computing a specific set of marginal probabilities efficiently. We demonstrate how these requested marginal probabilities can be computed efficiently for PCs in \cref{sec:fast-and-optimal}.

% Next, \cref{sec:tractability} confirms that the marginal probabilities requested by the high-level algorithms can be computed efficiently for PCs, which naturally leads to our proposed (de)compression algorithm. We conclude this section with empirical evaluations (\cref{sec:cmp-alg-eval}).

% In the following, we answer the above question in its affirmative. Specifically, we theoretically justify that compression and decompression are tractable and practical for (structured-)decomposable PCs (\cref{sec:tractability}), and provide an efficient (de)compression algorithm based on rANS \citep{duda2013asymmetric} (\cref{sec:rANS}). We conclude this section with empirical evaluations (\cref{sec:cmp-alg-eval}).






% \begin{proof}
% We start by providing some intuitions to \cref{thm:st-dec-pc-compress} that help illustrate the speedup from $\bigO(K \!\cdot\! \abs{\p})$ (\cf \cref{thm:dec-pc-compress}) to $\bigO(\log (K) \!\cdot\! \abs{\p})$ when structured-decomposability is additionally satisfied. The key to this speedup is the observation that part of the computation of the $K$ marginal probabilities in \cref{eq:cdf-breakdown} can be cached and reused. Suppose we want to compute $F_{\prec_{\pi}} (\x)$ given the PC shown in \cref{fig:sd-pc-compression}(a). By choosing a good variable order $\pi$, this computation can be significantly simplified. First, consider using a relatively bad variable order $X_1, X_2, X_3$ (\cref{fig:sd-pc-compression}(b)). To compute $\p(X_1 \!<\! x_1)$ (the first term in \cref{eq:cdf-breakdown}), we only need to evaluate the two input units correspond to $X_1$ (colored blue), and use the pre-computed top-down probabilities\footnote{Intuitively, the top-down probabilities represent the ``weight'' of each node to the final marginal probability. See \cref{sec:top-down-prob} for an $\bigO(\abs{\p})$ algorithm that compute this quantity for every PC unit.} of both units to weigh the probabilities of the two input units. We do not need to evaluate other nodes since they will either have probability $1$ or only contain information already cached in the top-down probabilities. Next, when computing the second term $\p(X_1 \!=\! x_1, X_2 \!<\! x_2)$, as illustrated in \cref{fig:sd-pc-compression}, we can reuse the evaluated probabilities of the two input units for $X_1$ (\ie the blue units), and only need to evaluate PC units colored in purple. The same scheme can be used when computing the other terms. As a result, we only need to evaluate 20 PC units in total to compute $F_{\prec_{\pi}} (\x)$, compared to $3 \abs{\p} \!=\! 39$ units required by the naive approach.

% As demonstrated in the previous example, even without a careful choice of variable order, we can significantly simplify computation cost by only evaluating the necessary PC units. We now show that with an \emph{optimal} choice of variable order $\pi$, the computation cost can be further reduced. Consider using variable order $X_3, X_2, X_1$, as shown in \cref{fig:sd-pc-compression}(c), we only need to evaluate $2 \!+\! 6 \!+\! 5 \!=\! 13$ PC units in total. This optimal variable order is the key to guarantee $\bigO(\log (K) \!\cdot\! \abs{\p})$ computation time, and showing this optimal variable order always exists is a central part of this proof.

% Next, we provide a high-level sketch of the proof, and defer technical details to \cref{sec:proof-sd-pc}. The proof consists of two main parts. First, we give a construction to compute the optimal variable order $\pi^{*}$ for any smooth and structured-decomposable PC. Next, we prove that following $\pi^{*}$, $F_{\prec_{\pi^{*}}} (\x)$ can be computed by evaluating no more than $\bigO(\log (K) \!\cdot\! \abs{\p})$ PC units.
% \end{proof}

% \begin{thm}
% \label{thm:dec-pc-neg-res}
% There exists a smooth and decomposable PC $\p$ defined on $K$ categorical variables, such that for any variable order $\pi$, computing $F_{\prec_{\pi}} (\x)$ takes $\Omega (K \!\cdot\! \abs{\p})$ time. \anji{Add proper assumptions on how the number is computed.}
% \end{thm}

==========

Range-based compression algorithms such as Arithmetic Coding \citep{rissanen1976generalized}, Range Encoding \citep{martin1979range}, and rANS \citep{duda2013asymmetric} are widely used by neural compression methods thank to their simplicity and optimality. Despite their different implementations, range-based compression algorithms are based on the following high-level idea: given a probability distribution $\p(\X)$, they (implicitly) assign every instance $\x \!\in\! \val(\X)$ with a range $[r_l (\x), r_h (\x)) \!\subseteq\! [0,1)$ such that (i) size of the range is proportional to the sample's probability: $r_h(\x) \!-\! r_l (\x) \!\propto\! \p(\x)$ and (ii) the ranges for $\val(\X)$ are non-overlapping and sum up to one: $\sum_{\x\in\val(\X)} (r_h (\x) \!-\! r_l (\x)) \!=\! 1$. Then, these algorithms compress $\x$ by finding the shortest codeword that can uniquely represent $[r_l (\x), r_h (\x))$. Since finding the shortest codeword given a range takes negligible time \citep{rissanen1976generalized}, the time complexity of these algorithms is determined by the efficiency of computing $r_l (\x)$ and $r_h (\x)$.

To satisfy its properties, the ranges $[r_l (\x), r_h (\x)) \,(\forall \x \!\in\! \val(\X))$ must have the following form
    {\setlength{\abovedisplayskip}{0.4em}
    \setlength{\belowdisplayskip}{-1.0em}
    \begin{align}
        r_l (\x) := \sum\nolimits_{\x'\prec\x} \p(\x'), \qquad r_h (\x) := r_l (\x) + \p(\x),
        \label{eq:def-range}
    \end{align}}
    
\noindent where $\prec$ is any ordering relation over $\val(\X)$. To compress a sample $\x$, a naive way is to compute $r_{l} (\x)$ and $r_{h} (\x)$, and then convert the range into a codeword with e.g. Arithmetic Coding. However, this is impractical due to the numerical errors of floating point numbers --- we often do not have enough precision to represent $r_{l} (\x)$ and $r_{h} (\x)$. To overcome this problem, we can break down $\p(\x)$ into $K \!:=\! \abs{\X}$ conditional probabilities and compress them sequentially:
    {\setlength{\abovedisplayskip}{0.4em}
    \setlength{\belowdisplayskip}{-0.8em}
    \begin{align}
        \p (\x) = \prod\nolimits_{i=1}^{K} \p (X_{\pi_{i}} = x_{\pi_{i}} \, | \, \{X_{\pi_{j}} = x_{\pi_{j}} \}_{j=1}^{i-1} ).
        \label{eq:compress-breakdown}
    \end{align}}
    
\noindent where $\pi$ defines a random variable order of $\X$, \ie the $j$th variable in the order defined by $\pi$ is $X_{\pi_j}$. As we will proceed to show in \cref{sec:fast-and-optimal}, an optimal choice of variable order is crucial to guarantee computational efficiency in the proposed (de)compression algorithm for PCs.

Following \cref{eq:def-range}, the range $[r_{l,i} (\x), r_{h,i} (\x))$ for the $i$th term in \cref{eq:compress-breakdown} has the following form
    {\setlength{\abovedisplayskip}{0.4em}
    \setlength{\belowdisplayskip}{-1.0em}
    \begin{align}
        r_{l,i} (\x) & := \sum\nolimits_{x' < x_{\pi_i}} \p (X_{\pi_{i}} \!=\! x' \, | \, \{X_{\pi_{j}} \!=\! x_{\pi_{j}} \}_{j=1}^{i-1} ) = \p (X_{\pi_{i}} \!<\! x_{\pi_{i}} \, | \, \{X_{\pi_{j}} \!=\! x_{\pi_{j}} \}_{j=1}^{i-1} ), \label{eq:dec-ranges-1} \\
        r_{h,i} (\x) & := r_{l,i} (\x) + \p (X_{\pi_{i}} \!=\! x_{\pi_{i}} \, | \, \{X_{\pi_{j}} \!=\! x_{\pi_{j}} \}_{j=1}^{i-1} ), \label{eq:dec-ranges-2}
    \end{align}}
    
\noindent where we choose the ordering relation $\prec$ to be $<$. Once having all $K$ ranges $[r_{l,i} (\x), r_{h,i} (\x))$, we can convert them into a bitstring representing the codeword of $\x$ using rANS. Note that since (i) we need to decompress the variables following order $\pi$ and (ii) rANS is stack-based, we need to encode the $K$ ranges in reverse order (\ie from $[r_{l,K}(\x), r_{h,K}(\x))$ to $[r_{l,1}(\x), r_{h,1}(\x))$).

The decompressor works by sequentially decoding the variables following order $\pi$. In the $i$th iteration, we have already obtained $\{x_{\pi_{j}}\}_{j=1}^{i-1}$ and want to decode $x_{\pi_{i}}$. To do that, we first extract a number $z$ (termed \emph{slot} in the rANS literature) in the current bitstring that is guaranteed to lie in the range $[r_{l,i} (\x), r_{h,i} (\x))$ (decompressor does not know this range for now). Then, binary search over variable $X_{\pi_{i}}$ is performed to find $x_{\pi_{i}}$ such that $z$ lies in its range: $r_{l,i}(\{x_{\pi_{j}}\}_{j=1}^{i-1}, x_{\pi_i}) \!\leq\! z \!<\! r_{h,i}(\{x_{\pi_{j}}\}_{j=1}^{i-1}, x_{\pi_i})$. Finally, we pop the encoded codeword representing $[r_{l,i} (\x), r_{h,i} (\x))$ from the bitstring and move on to decode the next variable.

The main bottleneck for both the compressor and the decompressor is the computation cost of $\{r_{l,i}(\x), r_{h,i}(\x)\}_{i=1}^{K}$.\footnote{Due to the additional complexity of performing binary search, for categorical variables $\X$ with $C$ categories, the decompressor needs to compute each of the $K$ ranges given at most $\lceil \log C \rceil$ different assignments $\x$.} Since every conditional probability in \cref{eq:dec-ranges-1,eq:dec-ranges-2} can be represented as the quotient of two marginal probabilities, computing $\{r_{l,i}(\x), r_{h,i}(\x)\}_{i=1}^{K}$ is equivalent to calculating the two following sets of marginal probabilities:
    {\setlength{\abovedisplayskip}{0.4em}
    \setlength{\belowdisplayskip}{-1.0em}
    \begin{align*}
        F_{\pi} (\x) \!:=\! \big \{ \p ( X_1 \!=\! x_1, \!\cdots\!, X_i \!=\! x_i) \big \}_{i=1}^{K}, \quad G_{\pi} (\x) \!:=\! \big \{ \p ( X_1 \!=\! x_1, \!\cdots\!, X_{i-1} \!=\! x_{i-1}, X_i \!<\! x_i) \big \}_{i=1}^{K}.
    \end{align*}}

% In this section, we turn \cref{thm:st-dec-pc-compress} into an efficient practical algorithm for (de)compression. A naive algorithm would be to first compute $F_{\prec_{\pi^{*}}} (\x)$ and $\p (\x)$, and then use Arithmetic Coding to convert the range $[F_{\prec_{\pi^{*}}} (\x), F_{\prec_{\pi^{*}}} (\x) \!+\! \p (\x))$ into a codeword. However, this is impractical due to the numerical errors of floating point numbers --- we do not have enough precision to represent $F_{\prec_{\pi^{*}}} (\x)$. 

% To overcome this problem, we break down $\p (\x)$ into $K$ conditional probabilities and compress them with a stream-based rANS algorithm by computing a range for each of the $K$ probability terms:
    
% As demonstrated in \cref{alg:compress}, to compress a sample $\x$, we first compute a range $[l[i], h[i])$ for each of the $K$ conditional probabilities in \cref{eq:compress-breakdown} (lines 5-7). As a corollary of \cref{thm:st-dec-pc-compress}, we show in \cref{sec:alg-efficiency} that computing all $K$ ranges take $\bigO (\log (K) \!\cdot\! \abs{\p})$ time. We then encode the ranges into a bitstring using rANS (lines 8-10). Note that since (i) we need to decompress the variables following the order $\pi^{*}$ and (ii) rANS is stack-based, we need to encode the $K$ ranges in reverse order (\ie from $K$ to $1$). 

% As illustrated in \cref{alg:decompress}, the decompressor works by sequentially decoding the variables following order $\pi^{*}$. In the $i$th iteration (decoding $X_{\pi^{*}_{i}}$), in line 5, we first extract a number $z$ representing the range $[l[i], h[i])$ (\cf lines 6-7 of \cref{alg:compress}), and then use binary search to find the correct $x_{\pi^{*}_{i}}$ (line 6). For categorical variables with $C$ categories, the binary search runs for at most $\lceil \log C \rceil$ times. Due to this additional complexity, decompression will be slower than compression. Finally, in line 7, we update the bitstring $b$ with rANS by popping the encoded number representing $[l(i), h(i))$.

% \section{Background}

% This section introduces relevant background on PCs (\cref{sec:background-pc}) and lossless compression (\cref{sec:background-compression}).

% We sometimes abbreviate structured-decomposability by SD. Although the above-defined structural properties may seem restrictive, we will show in the following sections that we can learn complex PCs that satisfy \cref{defn:smoothness,defn:decomposability,defn:st-decomposability} while still achieve high compression ratios.

% Denoted $\p_{\mathrm{down}} (n)$, the top-down probability of PC unit $n$ is designed to represent the ``weight'' of $n$ contributed to the final marginal probability. Back to our example, denote the two blue input units as $n_1$ and $n_2$, respectively. The top-down probabilities are designed such that $\p(X_1 \!<\! x_1) \!=\! \sum_{i=1}^{2} \p_{\mathrm{down}} (n_i) \!\cdot\! \p(n_i)$, where $\p(n_i)$ is the evaluated probability of $n_i$. 

% : (i) assign probability $1$ to $n$ and all its non-ancestor units whose scope is different from $\phi(n)$; (ii) assign probability $0$ to all non-ancestor units of $n$ whose scope is identical to $\phi(n)$; $\p_{\mathrm{down}} (n)$ is defined as the resultant probability of the root node by evaluating ancestors of $n$ following \cref{eq:pc-def}. Intuitively, the top-down probabilities represent the ``weight'' of each node to the final marginal probability. Back to our example, denote the two blue input units as $n_1$ and $n_2$.

% Since computing the likelihood $\p(\x)$ is tractable for most probabilistic models, we focus on the tractability of $r_l (\x)$ (\cref{eq:def-range}), as it characterizes the tractability of (de)compression. That is, the time complexity of (de)compression and computing $r_l (\x)$ will be roughly the same.\footnote{This is true because other steps in these entropy coding algorithms (Arithmetic Coding, Range Encoding, and rANS) only take time proportional to the length of the codeword.} To begin with, we establish a positive result showing that compressing samples \wrt smooth and decomposable PCs can be done in $\bigO(K \!\cdot\! \abs{\p})$ time, where $K$ is the number of variables.

% \begin{thm}
% \label{thm:dec-pc-compress}
% For a smooth and decomposable PC $\p$ defined on $K$ categorical variables $\X$ and a sample $\x$, computing $F_{\prec} (\x) \!:=\! \sum_{\x' \prec \x} \p(\x')$ takes $\bigO(K \!\cdot\! \abs{\p})$ time. Here $\prec$ defines an ordering relation over $\val(\X)$: $\x' \!\prec\! \x$ iff there exists $i \!\in\! [K]$ s.t. (i) $\forall j \!\in\! [i\!-\!1]$, $x'_{j} \!=\! x_{j}$ and (ii) $x'_i \!<\! x_i$.
% \end{thm}

% \begin{proof}
% The key to this proof is the observation that $F_{\prec}(\x)$ can be broken down into the sum of $K$ marginal probabilities:
%     {\setlength{\abovedisplayskip}{0.0em}
%     \setlength{\belowdisplayskip}{-0.6em}
%     \begin{align}
%         F_{\prec} (\x) = F_{\prec} (x_1 x_2 \cdots x_K) & = \sum_{i=1}^{K} \p(\underbrace{X_1 \!=\! x_1, \cdots, X_{i-1} \!=\! x_{i-1}}_{i - 1 \,\text{variable assignments}}, X_{i} \!<\! x_{i}).
%         \label{eq:cdf-breakdown}
%     \end{align}}

% We now demonstrate that each of the $K$ terms in \cref{eq:cdf-breakdown} can be computed in $\bigO(\abs{\p})$ time, rendering the computation time of $F_{\prec} (\x)$ to be $\bigO(K \!\cdot\! \abs{\p})$. Specifically, computing the $j$th term in \cref{eq:cdf-breakdown} consists of two steps: (i) assign probabilities to PC input nodes following the given variable assignments (assign probability $1$ if the corresponding variable is not assigned);\footnote{For every input unit $n$ whose corresponding variable has an inequality assignment, simply assign the cumulative probability: $\p_{n} (X_i \!<\! x_i) \!=\! \sum_{a=1}^{x_i-1} \p_{n} (X_i \!=\! a)$.} (ii) follow \cref{eq:pc-def} to compute the probability of every sum and product unit. The $j$th probability in \cref{eq:cdf-breakdown} will be the value of the PC's root node. Correctness of this computation has been proved for all smooth and decomposable PCs \citep{choiprobabilistic,poon2011sum}.
% \end{proof}

% The main problem for performing compression with smooth and decomposable PCs is the linear dependence on $K$, since the number of variables could easily reach several hundreds in many practical datasets. While one may hope that a better choice of $\prec$ may lead to more efficient algorithms, the following theorem demonstrates that this is impossible in a general sense. Before stating the formal result, we first define a class of binary relations.

% \begin{defn}
% Define $\pi$ as a random variable order over a set of variables $\X \!:=\! \{X_i\}_{i=1}^{K}$, that is, the $j$th variable in the order defined by $\pi$ is $X_{\pi_{j}}$. For every variable order $\pi$, we define binary relation $\prec_{\pi}$ as follows: $\x' \prec_{\pi} \x$ iff there exists $j \!\in\! [K]$ s.t. (i) $\forall k \!\in\! [j\!-\!1], x'_{\pi_{k}} \!=\! x_{\pi_{k}}$ and $x'_{\pi_{j}} \!=\! x_{\pi_{j}}$.
% \end{defn}

% We are now ready to state our negative result.

% Proof is provided in \cref{sec:proof-pc-neg-res}. Although $\prec_{\pi}$ is only a sub-class of all ordering relations $\prec$, if $\X$ are categorical variables, we conjecture that for every $\prec$ that is not equivalent to any $\prec_{\pi}$,\footnote{$\prec$  and $\prec_{\pi}$ are equivalent if they are made identical by swapping the ordering of categories of each variable.} $F_{\prec} (\x)$ is generally harder to compute since it cannot be represented as the sum of $K$ marginal probabilities.

% Structured-decomposability is the key to overcome the linear dependence on $K$. In the following, we will show that (de)compression with a smooth and structured-decomposable PC only requires $\bigO (\log (K) \!\cdot\! \abs{\p})$ time. We first give an additional definition.

% The above equality constraint may seem restrictive at a first glance. However, we highlight that (i) this is used to simplify the proof of \cref{thm:st-dec-pc-compress}, and the theoretical result will hold as long as the equation holds approximately; (ii) most existing PC structures such as HCLTs, EiNets, and RAT-SPNs are balanced (see \cref{sec:pc-balanced} for justifications). We are ready to present the positive result.

This section first introduces Hidden Chow-Liu Tree (HCLT), an expressive PC model that is smooth and structured-decomposable (\cref{sec:hclt}). We then briefly review the parameter learning algorithm for HCLTs (\cref{sec:hclt-param}) and empirically compare its generative learning performance with recent neural compression models (\cref{sec:hclt-eval}).

\subsection{Parameter Learning}
\label{sec:hclt-param}

Following recent advances in PC training \citep{peharz2016latent,dang2021juice}, we use the Expectation Maximization (EM) \citep{dempster1977maximum} algorithm to learn PC parameters. Specifically, we adopt the forward and backward algorithm introduced in \citet{liu2021tractable} to compute the \emph{expected flow} of every edge $(n,c)$, and update sum and input unit parameters using these flows \citep{ChoiAAAI21}. Please refer to \cref{sec:hclt-learning-details} for more details.

The construction process of an HCLT is illustrated in \cref{fig:hclt}. Suppose we are given a dataset $\data$ where each sample consists of 4 features $\{X_i\}_{i=1}^{4}$. We first learn a CLT using $\data$, which is done by finding the maximum spanning tree over the complete graph of variables with edges weighted by the corresponding empirical pair-wise mutual information. The original undirected CLT is transformed to a directed one by choosing the node at the graph center as the root node. A Probabilistic Graphical Model (PGM) \citep{koller2009probabilistic} representation of the learned CLT is shown in \cref{fig:hclt}(a).

Define $\{Z_i\}_{i=1}^{4}$ as a set of hidden variables that will be formally defined later. To improve expressiveness, hidden variables are added to the CLT in the following two steps: (i) replace observed variables $X_i$ by their corresponding hidden variables $Z_i$ (\cref{fig:hclt}(b)), and (ii) connect hidden variables $Z_i$ with the corresponding observed variables $X_i$ by directed edges. This leads to the PGM representation illustrated in \cref{fig:hclt}(c). 

We are now left with the final step of compiling the PGM representation of the model into an equivalent PC. Before doing this, we formally define the hidden variables $\{Z_i\}_{i=1}^{4}$ as categorical variables with $M$ categories, where $M$ is a hyperparameter. As demonstrated in \cref{alg:compile-hclt}, we incrementally compile every PGM node into an equivalent PC unit though a bottom-up traverse (line 5) of the PGM. Specifically, leaf PGM nodes corresponding to observed variables $X_i$ are compiled into PC input units of $X_i$ (line 6), and inner PGM nodes corresponding to hidden variables are compiled by taking products and sums (implemented by product and sum units) of its child nodes' PC units (lines 8-10). Since every image pixel can be regarded as a categorical variable with value ranging from 0 to 255, we use categorical input units with 256 categories in all PCs unless stated otherwise. \cref{fig:hclt}(d) demonstrates the result PC after running \cref{alg:compile-hclt} with the PGM in \cref{fig:hclt}(c) and $M=2$.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\textwidth]{iclr2022/figures/fig-hclt-mnist.pdf}
    \vspace{-1.0em}
    \caption{Bits-per-dim for HCLTs with different number of parameters on MNIST.}
    \label{fig:hclt-mnist}
\end{figure}

% Despite achieving state-of-the-art results on various tasks such as generating high-quality images, the performance of deep generative models is hindered when applied to lossless compression. For example, due to their inability to tractably compute sample likelihood, Variational Autoencoder-based compression algorithms suffer from very bad single-sample compression ratios. To overcome such problems, we use statistical models that permit efficient computation of marginal probabilities, an advantageous property when performing lossless compression. Specifically, we use Probabilistic Circuits (PCs), a class of neural networks that support efficient marginalization, as backbone models and develop compression and decompression algorithms that both have time complexity $\bigO(\log(K) \!\cdot\! \abs{\p})$, where $\abs{\p}$ is the model size and $K$ is the number of variables. Empirically, our PC-based (de)compression algorithm runs 5-20x faster than state-of-the-art neural compression algorithms while achieving similar bit-rates. Furthermore, by scaling up the structure and learning pipeline of PCs, we achieved state-of-the-art results on non-natural-image datasets such as MNIST. By replacing mutually-independent latent variables in Flow models with expressive PCs, we further achieved new state-of-the-art on natural image datasets such as sub-sampled ImageNet.

% \anji{Neural networks have been successful in generative modeling.}
% \anji{However, there are tasks not very suitable for them.}
% \anji{Lossless compression is one example, since our end goal is to learn distributions on discrete data.}
% \anji{There has been two types of approaches to fix this problem: (i) learn discrete distributions (\eg IDF), and (ii) apply quantization (\eg LBB).}
% \anji{Point out their respective problems.}

% \anji{We therefore seek models with the following properties: (i) , (ii), ...}

% \section{An Alternative Way to Model Complex Distributions}

% Deep Generative Models (DGMs) such as Flow-based models \citep{dinh2014nice}, Variational Autoencoders \citep{kingma2013auto}, and Generative Adversarial Networks \citep{goodfellow2014generative} are based on the simple yet effective idea of transforming simple prior distributions (\eg multi-variate Gaussian) into complex distributions representing the data (\eg images). Although it is widely believed that DGMs can transform simple prior distributions into the target very well given sufficient neural network capacity, it has been widely observed that using more complicated priors such as multi-modal distributions \citep{hoogeboom2019integer,johnson2016composing} and stochastic processes \citep{nalisnick2016stick,casale2018gaussian} lead to better performance.

% Therefore, to improve generative modeling performance, one can either design better prior-to-data transformations or learn better prior distributions.\footnote{Here, we refer to a broader sense of ``prior'' distributions, which include not only fixed and simple distributions (\eg Gaussian) but also probabilistic models (\eg Bayesian Networks).} However, the latter idea has been largely unexplored in the context of compression due to two main reasons: (i) the lack of expressive probabilistic models, and (ii) the inefficiency of performing (de)compression on these models. To better understand the second reason, suppose we have learned a distribution $\p_{\params}(\X)$ given samples $\{\x^{(i)}\}_{i=1}^{N}$. To compress a sample $\x$ with arithmetic coding \citep{witten1987arithmetic}, we need the cumulative probability over $\x$, \ie $\int_{\x' \preceq \x} \p_{\params}(\x') d \x'$, where $\preceq$ defines an arbitrary ordering relation over pair of instances in $\val(\X)$ (this claim is justified in \cref{sec:tractability}). This quantity is hard to compute unless highly simplified assumptions are made. For example, modern DGMs assume the (prior) variables $\X \!:=\! \{X_1,\dots,X_k\}$ are mutually independent, rendering the cumulative probability factorizable.

% In this paper, we aim to solve both issues with Probabilistic Circuits (PCs) \citep{choiprobabilistic}, a class of expressive Tractable Probabilistic Models (TPMs). First, we improve model expressiveness by pushing further recent breakthroughs in large-scale training \citep{dang2021juice} and model design \citep{peharz2020einsum,liu2021tractable} of PCs. As a result, we achieved good compression rates on many datasets with or without the help of additional neural network based transformation layers. Second, by leveraging PCs' ability to efficiently compute marginal probabilities, we develop efficient theoretically-grounded (de)compression algorithms that are 10x faster than DGMs that achieve similar compression rate.

% \section{Overview of Our Methods and Results}
% \label{sec:overview}

Next, we focus on efficiency. As shown in the last two columns of \cref{tab:cmp-decmp-time}, the compression time of PCs (\ie HCLT, $M \!=\! 16$) with better codeword bpd is over 20x faster than IDF and BitSwap. Although decompression is slower for PCs due to the additional complexity of the binary search, it is still 10x faster than IDF and BitSwap. Note that the superior computation cost is not a result of smaller model size because the adopted PCs have more parameters than BitSwap. See \cref{sec:cmp-decmp-exp-details} for more details.

Autoregressive models, Flow models, and VAEs are three classes of expressive DGMs. In the context of compression, autoregressive models are only used in limited circumstances due to their high decompression time \citep{child2019generating}. On the other hand, (de)compression with VAEs and Flow models only requires a single evaluation of the model. In addition to the adopted baselines, there has been many work on improving the expressiveness of VAE- \citep{townsend2019hilloc} and Flow-based \citep{van2020idf++,zhang2021ivpf} compression models. In terms of compression methods, Bits-back coding is a popular approach to improve the expected codeword length at the expense of bad single-sample compression ratio \citep{ho2019compression,townsend2018practical}.

We empirically evaluate HCLTs by comparing with density estimators based on discrete Flows (\ie IDF \citep{hoogeboom2019integer}) and hierarchical VAEs (\ie BitSwap \citep{kingma2019bit}). First, we compare density estimation performance (in bits-per-dim) on 5 datasets --- MNIST \citep{deng2012mnist}, FashionMNIST \citep{xiao2017fashion}, and the Letter and ByClass split of EMNIST \citep{cohen2017emnist}. As shown in \cref{tab:hclt-lls}, HCLT out-performs IDF and BitSwap on 4 and 3 datasets, respectively. While we were not able to obtain competitive performance on natural image datasets such as CIFAR10 with HCLTs, as we will elaborate in \cref{sec:pc+flow}, we can improve over IDF on natural image datasets by replacing its mutually independent latent variables with expressive PCs that can be jointly trained with the Flow model.

Next, we examine the succinctness (\ie \# parameters vs. bpd) on MNIST. As a baseline, the adopted IDF and BitSwap models have 24,175,272 and 2,839,636 parameters, respectively. As illustrated in \cref{fig:hclt-mnist}, HCLTs are both expressive and succinct --- an HCLT with 88,160 parameters already achieved $1.43$ bpd, and by increasing the model size to over 7 millions, HCLTs were able to achieve $1.20$ bpd. Additionally, an HCLT with 1,430,080 parameters achieved the same performance compared to BitSwap, which contains twice as many parameters. See \cref{sec:hclt-exp-details,sec:idf-bitswap-details} for more experiment details on HCLT and the baselines, respectively.

Motivated by the observation that more expressive prior distributions lead to better generative performance in Flow models, we propose to replace the mutually-independent priors variables with PCs over the same set of variables. Specifically, as illustrated in \cref{fig:pc-flow-model}, we use a PC to represent the probability of each of the $k$ sets of latent variables in IDF \citep{hoogeboom2019integer}, a discrete Flow model. Given a sample $\x$, the log-likelihood of the model is the sum of the $k$ PCs' output log-likelihood: $\log \p_{\params}(\x) \!=\! \sum_{i=1}^{k} \log \p(\z_i \mid \x)$. This PC+IDF model can be trained end-to-end since PCs are differentiable and can pass gradients to the IDF. \anji{Empirical result}

Compression can be done by first obtaining the latent variables $\{\z_{i}\}_{i=1}^{k}$ and then compress them using the PCs and \cref{alg:compress}. Decompression proceeds by iteratively decompress the set of variables $\z_k, \dots, \z_1, \x$ with \cref{alg:decompress} and gradually evaluate the IDF in reverse order.

\subsection{Proof of Theorem~\ref{thm:dec-pc-neg-res}}
\label{sec:proof-pc-neg-res}

We start by constructing an example PC. Suppose there are $k$ categorical variables. We first construct $k$ structured-decomposable PCs following the $k$ vtrees illustrated in \cref{fig:bad-dec-pc}, respectively. One way to construct such PCs is by treating the vtrees as a PGM and invoke \cref{alg:compile-hclt}. Denote the $k$ resultant PCs as $\p_1, \dots, \p_k$, respectively. Next, we put a sum unit over the $k$ structured-decomposable PCs $\{\p_j\}_{j=1}^{k}$, and denote the resultant PC as $\p$. W.l.o.g. we assume the parameters of the root sum unit are all $\frac{1}{k}$.

Suppose the $k$ PCs $\{\p_j\}_{j=1}^{k}$ have identicle size, then it follows that for every PC $\p_j$, each of its vtree node corresponds to $\Theta (\frac{\abs{\p}}{K^2})$ PC units.

For $\p$, we want to compute
    \begin{align*}
        F_{\prec_{\pi}} (\x) & = \sum_{i=1}^{k} \p(X_{\pi_{1}} \!=\! x_{\pi_{1}}, \dots, X_{\pi_{i-1}} \!=\! x_{\pi_{i-1}}, X_{\pi_{i}} \!<\! x_{\pi_{i}}) \\
        & = \frac{1}{k} \sum_{i=1}^{k} \sum_{j=1}^{k} \underbrace{\p_{j}(X_{\pi_{1}} \!=\! x_{\pi_{1}}, \dots, X_{\pi_{i-1}} \!=\! x_{\pi_{i-1}}, X_{\pi_{i}} \!<\! x_{\pi_{i}})}_{\overset{\mathrm{def}}{=} G_{\pi}(i,j)}.
    \end{align*}
For any $i \geq 2$, and any variable order $\pi$, in order to compute $\sum_{j=1}^{k} G_{\pi}(i,j)$, we need to evaluate PC units corresponding to at least $i \!\cdot\! \lfloor \frac{k}{2} \rfloor \!=\! \lfloor \frac{i \cdot k}{2} \rfloor$ vtree nodes. The reason is elaborated in the following. First, for every variable $X$ in $\{X_{\pi_{l}}\}_{l=1}^{i-1}$, there are at least $\lfloor \frac{k}{2} \rfloor$ PCs in $\{\p_j\}_{j=1}^{k}$ such that the variable $X$ is on top of $X_{\pi_{i}}$ in the PC's vtree. Thus, there are in total $i \!\cdot\! \lfloor \frac{k}{2} \rfloor$ variables-PC pair $(X,\p_l)$ such that $X$ appears on top of $X_{\pi_{i}}$ in the vtree of $\p_l$.

Next, for each $\q \!\in\! \{\p_{j}\}_{j=1}^{k}$, if there are $l$ variables in $\{X_{\pi_{l}}\}_{l=1}^{i-1}$ that appears ``above'' $X_{\pi_{i}}$ in its vtree, we need to evaluate PC units correspond to $l$ vtree nodes in order to compute $G_{\pi}(i,j)$, since we need to at least evaluate (i) the parent of vtree node $X_{\pi_{i}}$ and (ii) the parent of vtree node $X$, where $X$ appears ``above'' $X_{\pi_{i}}$. Combining the argument in the previous paragraph, we need to evaluate at least $i \!\cdot\! \lfloor \frac{k}{2} \rfloor$ vtree nodes in order to compute $\sum_{j=1}^{k} G_{\pi} (i,j)$. Therefore, we need to evaluate at least 
    \begin{align*}
        \sum_{i=2}^{k} i \!\cdot\! \left \lfloor \frac{k}{2} \right \rfloor > \left \lfloor \frac{k (k-1)^2}{4} \right \rfloor
    \end{align*}
\noindent vtree nodes to compute $F_{\prec_{\pi}} (\x)$. This is equivalent to at least $\Theta(K \!\cdot\! \abs{\p})$ PC units (since each vtree node corresponds to $\Theta (\frac{\abs{\p}}{K^2})$ PC units).

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{iclr2022/figures/fig-bad-dec-pc.pdf}
    \caption{A construction of smooth and decomposable PC that is used to prove \cref{thm:dec-pc-neg-res}.}
    \label{fig:bad-dec-pc}
\end{figure}

\subsection{Efficiency of Algorithms~\ref{alg:compress} and \ref{alg:decompress}}
\label{sec:alg-efficiency}

Recall from \cref{sec:compression-alg} that the definition of $l[i]$ and $h[i]$ are given by:
    \begin{align*}
        l[i] & := \p \big (X_{\pi^{*}_{i}} \!<\! x_{\pi^{*}_{i}} \mid \{X_{\pi^{*}_{j}} \!=\! x_{\pi^{*}_{j}} \}_{j=1}^{i-1} \big ) = \frac{\p \big  (\{X_{\pi^{*}_{j}} \!=\! x_{\pi^{*}_{j}} \}_{j=1}^{i-1}, X_{\pi^{*}_{i}} \!<\! x_{\pi^{*}_{i}} \big )}{\p \big (\{X_{\pi^{*}_{j}} \!=\! x_{\pi^{*}_{j}} \}_{j=1}^{i-1} \big )}, \\
        h[i] & := l[i] + \p \big (X_{\pi^{*}_{i}} \!=\! x_{\pi^{*}_{i}} \mid \{X_{\pi^{*}_{j}} \!=\! x_{\pi^{*}_{j}} \}_{j=1}^{i-1} \big ) = l[i] + \frac{\p \big  (\{X_{\pi^{*}_{j}} \!=\! x_{\pi^{*}_{j}} \}_{j=1}^{i} \big )}{\p \big (\{X_{\pi^{*}_{j}} \!=\! x_{\pi^{*}_{j}} \}_{j=1}^{i-1} \big )}.
    \end{align*}
According to \cref{thm:st-dec-pc-compress}, the following set of terms can be computed in $\bigO (\log (K) \!\cdot\! \abs{\p})$ time: 
    \begin{align}
        \left \{ \p \big (\{X_{\pi^{*}_{j}} \!=\! x_{\pi^{*}_{j}} \}_{j=1}^{i-1}, X_{\pi^{*}_{i}} \!<\! x_{\pi^{*}_{i}} \big ) \right \}_{i=1}^{K} \text{~and~} \left \{ \p \big (\{X_{\pi^{*}_{j}} \!=\! x_{\pi^{*}_{j}} \}_{j=1}^{i} \big ) \right \}_{i=1}^{K}.
        \label{eq:proof-computable-terms}
    \end{align}
Thus, $\{[l[i], h[i])\}_{i=1}^{K}$ can be computed in $\bigO (\log (K) \!\cdot\! \abs{\p})$ since they only consists of the terms in \cref{eq:proof-computable-terms}.

\subsection{Computing PC Top-down Probabilities}
\label{sec:top-down-prob}

The algorithm for computing the top-down probabilities of PC units is shown in \cref{alg:top-down-prob}. We use \cref{fig:sd-pc-compression}(b) as an example to demonstrate the use of the computed $\mathrm{top\_down\_prob}$. Suppose we want to compute $\p(X_1 < x_1)$, and we have evaluated the two input units correspond to variable $X_1$ (\ie the two blue units). Denote the two nodes as $n_1$ and $n_2$, respectively. $\p(X_1 < x_1)$ can be computed as follows
    \begin{align*}
        \p(X_1 < x_1) = \sum_{n\in\{n_1,n_2\}} \frac{\mathrm{top\_down\_prob}[n]}{\sum_{m\in\{n_1,n_2\}}\mathrm{top\_down\_prob}[m]} \cdot \p_{n} (X_1 < x_1).
    \end{align*}
The above equation can be directly generalized to compute other marginal probabilities by changing the set $\{n_1,n_2\}$ to the set of evaluated PC units whose parents are not evaluated.

\subsection{Details on the Adopted HCLTs}
\label{sec:hclt-exp-details}

We used two factors to control the size of HCLTs used in the experiment shown in \cref{fig:hclt-mnist} --- hyperparameter $M$ (the number of hidden categories, see \cref{sec:hclt}), and the sparseness of the categorical input units. In the following, we elaborate the second factor in detail.

Since each image pixel can be regarded as a categorical variable with 256 categories, the HCLTs used input categorical units each with 256 parameter representing the probability of each category. However, we found many of these parameters are useless due to their extremely small values after convergence (\eg $1e\!-\!7$). Therefore, after the training stage, we add a finetune stage where for each (categorical) input unit $n$, we force the smallest $\tau \%$ of parameters to be identicle, thus each input node only has $\lceil (1\!-\!\tau \%) \!\cdot\! 256 \rceil$ parameters. In our experiments we chose $M \!\in\! \{4, 12, 16, 20, 24, 28, 32\}$ and $\tau \!\in\! \{95, 90, 80, 60, 40, 20\}$.

\subsection{Experiment Details for Neural Compression Baselines}
\label{sec:idf-bitswap-details}

\paragraph{IDF} We ran all experiments with the code in the GitHub repo provided by the authors. We adopted an IDF model with the following hyperparameters: 8 flow layers per level; 2 levels; densenets with depth 6 and 512 channels; base learning rate $0.001$; learning rate decay $0.999$.

\paragraph{BitSwap} We ran all experiments using the following author-provided script: \url{https://github.com/fhkingma/bitswap/blob/master/model/mnist_train.py}.

\paragraph{BB-ANS} All experiments were performed using the following official code: \url{https://github.com/bits-back/bits-back}.

By combining \cref{alg:compute-marginals} with rANS (other streaming codes can also be used), our PC-based (de)compression algorithm is both fast and competitive. As we will proceed to show in \cref{tab:cmp-decmp-time}, a PC compressor took 59s to encode and decode 10,000 MNIST images while achieving 1.30 bits-per-dimension (bpd). In contrast, BitSwap \citep{kingma2019bit}, a neural compression algorithm that achieved competitive 1.31 bpd, took 904s ($\smallsim\!15$x slower) to encode and decode these images.

Specifically, compression algorithms start with an empty bitstream $b$ representing the initial interval $[0,1)$; while encoding symbol $x_i$, we first compute the following two quantities representing an interval:
    
\noindent  We drop the dependency on $x_1, \dots, x_{i-1}$ in $l_{i} (x_i)$ and $r_{i} (x_i)$ for notation simplicity. The computed interval $[l_{i} (x_i), h_{i} (x_i))$ is then used to refine the interval specified by $b$,

\ie $b$ is updated to encode $x_i$. Upon decoding, the symbols $\{x_i\}_{i=1}^{D}$ (define $D \!:=\! \abs{\X}$ as the number of features) are decoded sequentially: at iteration $i$, we decode variable $X_i$ by looking up its value $x$ such that $l_{i} (x)$ matches the subinterval specified by $b$ and $x_1,\dots,x_{i-1}$ \citep{rissanen1976generalized}; the decoded symbol $x_i$ is then used to compute the following conditional probabilities (\ie $l_{j}(x)$ for $j>i$). The main computation cost of both the encoding and decoding process comes from calculating $l_{i} (x)$ and $h_{i} (x)$.

\anji{Take AC as an example.... Other streaming codes such as .. also need to compute l and h}

\begin{rethm}[\ref{thm:st-dec-pc-compress}]
For a PC model $\p$ defined on $D$ variables $\X$, there exists a variable order over $\X$ that conforms this ordering \guy{what does it mean for an ordering to 'conform to this ordering'?} such that for all $\x$, computing $\{l_{i}(x_i), h_{i}(x_i)\}_{i=1}^{D}$ following \cref{alg:compute-marginals} takes $\bigO(\log(D) \cdot \abs{\p})$ time, where $\abs{\p}$ is the size of $\p$.
\vspace{-0.4em}
\end{rethm}

Once all intervals are calculated, the data can be en- or decoded autoregressively, involving a total coding cost of $\bigO(\log(D) \cdot \abs{\p} + D) = \bigO(\log(D) \cdot \abs{\p})$ since $|p|\geq D$ for PCs. 

A key to the efficiency of \cref{alg:compute-marginals} is the observation that we only need to evaluate the PC model partially in order to compute each conditional probability, which will be elaborated in \cref{sec:tractability}. Additionally, we highlight that \cref{alg:compute-marginals} is efficient only if an optimal variable order, which depends on the PC's architecture, is used. Thus finding and proving the existence of the optimal variable order is a key to ensuring the efficiency of the proposed (de)compressor.\guy{less is more? these details might confuse and not help}

Since good generative performance does not imply good compression performance, one may wonder if there exists a class of models currently overlooked by the compression community that ensures (i) good compression rates and (ii) tractable algorithms to efficiently encode and decode close to the model's theoretical rate estimate. This paper answers this question affirmatively and for the first time proposes Probabilistic Circuits (PCs) \citep{choiprobabilistic} for lossless compression.

In order to support efficient marginalization, PCs need to satisfy two \emph{structural properties} --- smoothness (\cref{defn:smoothness}) and decomposability (\cref{defn:decomposability}).\footnote{Sufficiency of the conditions are proved by \citet{poon2011sum}.} Both are properties of the (variable) \emph{scope} $\phi(n)$ of PC units $n$, that is, the collection of variables defined by all its descendent input units.

\begin{defn}[Smoothness]
\label{defn:smoothness}
A PC is smooth if for every sum unit $n$, its children have the same scope: $\forall c_1, c_2 \in \ch(n), \phi(c_1) = \phi(c_2)$.
\end{defn}

% \guy{I would much rather have a simpler basic readable theorem statement here saying: 
% \begin{rethm}[\ref{thm:st-dec-pc-compress}]
% Let $\x$ be a $D$-dimensional sample, and let $\p$ be a PC model of size $\abs{\p}$, as proposed in this paper.
% We then have that computing all quantities $\{l_{i}(x_i), h_{i}(x_i)\}_{i=1}^{D}$ takes $\bigO(\log(D) \cdot \abs{\p})$ time.
% Therefore, autoregressive en- or decoding of $\x$ takes $\bigO(\log(D) \cdot \abs{\p})$ time.
% \end{rethm}
% I don't think it makes sense right here to start talking about variable orders and Alg 2 and details that will be fleshed out later.
% Instead you can make a forward pointer: the properties of PCs that enable this complexity will be described in Section X, and the inference algorithm that achieves this complexity will later be shown as Alg 2.
% }

\anji{Outline of structure: (i) briefly describe fig. 2. (ii) state the purpose of the backbone marginalization algorithm (we want to compute .....). (iii) Naive algorithm (linear complexity). (iv) Proposed algorithm: we use a similar strategy as partial elimination, but we eliminate more units. This is the key to the log D improvement. (v) Elaborate the algorithm, and leave ``which nodes can be reused'' as a key question. (vi) Provide some hints using Fig. 2. (vii) Provide ingredients to give the formal theorem, and refer everything else to the appendix.}

the small PC model achieved 1.30 compression bits-per-dimension (bpd). Compared to BitSwap \citep{kingma2019bit}, which achieved a similar bitrate (1.31), our approach is $\smallsim \! 15$x faster in terms of en- and decoding speed. Furthermore, a larger PC model achieved a much better bitrate (1.24) while still being $\smallsim \! 4.5$x faster than BitSwap. 

Furthermore, a larger PC model achieved a much better bitrate while still being $\smallsim \! 4.5$x faster than the baselines.

% On the one hand, highly expressive probability models such as autoregressive neural networks \citep{Salimans2017PixeCNN,papamakarios2017masked} enjoy high compression ratios at the cost of slow runtime --- decoding a sample requires evaluating the model $D$ times, where $D$ is oftentimes several hundred in practical datasets.\footnote{
%     Note that high-resolution images can be generally compressed in patches.}
% On the other hand, adding strong independence assumptions in $\p$ (\eg $\X$ are mutually independent) makes $l_{i}(x)$ and $h_{i}(x)$ highly tractable. However, model expressiveness is greatly sacrificed.\footnote{
%     Flow-model-based neural compression algorithms adopt $\p$ defined on mutually independent latent variables (denoted $\Z$), and improve expressiveness by learning bijection functions between $\Z$ and $\X$ (\ie the input space). This is orthogonal to our approach of directly learn better $\p$. Furthermore, we can naturally integrate proposed expressive $\p$ with the bijection functions and achieve better performance as demonstrated in \cref{sec:pc+flow}.}

==> tikz/tikzlibrarypc.code.tex <==
% Copyright 2016 by Nicola Di Mauro and Antonio Vergari
%
% This file may be distributed and/or modified
%
% under the GNU General Public License.
%
% See the files LICENSE for more details.

\usetikzlibrary{chains}
%\usetikzlibrary{arrows}
\usetikzlibrary{calc}
\usepackage{pgfplots}
\usepackage{xparse}
%\usepackage{listofitems}

%\newif\iflabelleft

\newdimen\mywidth
\newdimen\myheight

\newcommand*{\IfStringInList}[2]{%
  \in@{,#1,}{,#2,}%
  \ifin@
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pgfmathdeclarefunction{gauss}{2}{%
  \pgfmathparse{1/(#2*sqrt(2*pi))*exp(-((x-#1)^2)/(2*#2^2))}%
}

% sum node style
\tikzstyle{sum} = [circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
minimum size=18pt, path picture={\draw [shorten >=3pt,shorten <=3pt] (path picture bounding box.south) -- (path picture bounding box.north); \draw [shorten >=3pt,shorten <=3pt] (path picture bounding box.west) -- (path picture bounding box.east);}, node distance=1]

% product node style
\tikzstyle{prod} = [circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
minimum size=18pt, path picture={\draw [shorten >=6pt,shorten <=6pt] (path picture bounding box.south east) -- (path picture bounding box.north west); \draw [shorten >=6pt,shorten <=6pt] (path picture bounding box.south west) -- (path picture bounding box.north east);}, node distance=1]

% \sumnode [tikz-options] {sum node name} 
\newcommand{\sumnode}[2][]{
  \node[sum, #1] (#2) {};
}

% \prodnode [tikz-options] {product node name} 
\newcommand{\prodnode}[2][]{
  \node[prod, #1] (#2) {};
}
\newcommand{\wprodnode}[3][]{
  \node[prod, #1] (#2) {$\color{#3}\times$};
}

% \maxnode [tikz-options] {max node name} 
\newcommand{\maxnode}[2][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {\scriptsize $max$};
}

% \emptynode [tikz-options] {generic node name}
\newcommand{\emptynode}[2][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {};
}

\newcommand{\varnode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt, minimum size=19pt, #1] (#2) {#3};
}

\newcommand{\varsqnode}[4][]{
  \node[rectangle, rounded corners=3pt,fill=white,draw=#4,inner sep=0pt,line width=0.6pt, minimum size=19pt, #1] (#2) {#3};
}

\newcommand{\evnode}[4][]{
  \node[circle,fill=#4,text=white,inner sep=0pt, minimum size=18pt, #1] (#2) {#3};
}

\newcommand{\evnodevar}[5][]{
  \node[circle,fill=#4,text=white,inner sep=0pt, minimum size=18pt,
  #1] (#2) {#3};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#5};
}

\newcommand{\bernode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, #1] (#2) {\tikz\draw circle (3pt);};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\bernodeleft}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, #1] (#2) {\tikz\draw circle (3pt);};
  \node[left=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\bernodedown}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, #1] (#2) {\tikz\draw circle (3pt);};
  \node[below=1pt of #2, yshift=1pt] (#2_vn) {#3};
}

\newcommand{\cbernodedown}[4][]{
  \node[circle,fill=white,draw=#4,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, #1] (#2) {\tikz\draw[draw=#4] circle (3pt);};
  \node[below=1pt of #2, yshift=1pt] (#2_vn) {\textcolor{#4}{#3}};
}

\DeclareDocumentCommand{\contnode}{o m m o}  
{%
  \IfNoValueTF{#4}
  {\contnodebelow[#1]{#2}{#3}}
  {\contnodeleft[#1]{#2}{#3}}
}

\newcommand{\contnodebelow}[3][]{  
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {           
          \begin{tikzpicture}
                \begin{axis}[
                no markers, scale only axis, domain=-4:4,samples=50, smooth,
                axis lines=none,
                height=10pt]
                \addplot [mark=none] {gauss(0,1)};
                \end{axis}
              \end{tikzpicture}};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\contnodeleft}[3][]{  
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {           
          \begin{tikzpicture} 
                \begin{axis}[
                no markers, scale only axis, domain=-4:4,samples=50, smooth,
                axis lines=none,
                height=10pt]
                \addplot [mark=none] {gauss(0,1)};
                \end{axis}
              \end{tikzpicture}};
  \node[left=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\catnode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=18pt, node distance=1, #1] (#2) {           
          \begin{tikzpicture} %these distributions look really distorted, and are the ones I want to include, inside the minipage
                \begin{axis}[
                no markers, scale only axis, domain=-4:4, smooth,
                axis lines=none,
                height=10pt]
                \addplot [mark=none] coordinates { (0,0) (0,10)};
                \addplot [mark=none] coordinates { (-1,0) (-1,7)};
                \addplot [mark=none] coordinates { (-2,0) (-2,3)};
                \addplot [mark=none] coordinates { (1,0) (1,5)};
                \addplot [mark=none] coordinates { (2,0) (2,8)};
                \end{axis}
            \end{tikzpicture}};
  \node[below=1pt of #2] (#2_vn) {#3};
}


% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [-,line width=0.6pt,#1] (\y) ;%
    } ;
  } ;
}

\newcommand{\cedge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \draw[-,#1] (\x)+(0,-9pt) -- ($(0,9pt)+(\y)$);
      % \path ([yshift=9pt]\x) edge [-,#1] ([yshift=9pt]\y) ;%
    } ;
  } ;
}

\newcommand{\upedge}[3][]{
  \path (#2) edge [line width=1pt,->,>=stealth,#1] (#3);
}

\newcommand{\ledge}[4][]{
  \path (#2) edge [line width=1pt,->,>=stealth,#1,edge label=#4] (#3);
}

\newcommand{\weigedge}[4][]{
  \draw[line width=0.6pt,-,#1] (#2) edge node [midway,line width=0.6pt,#1] {#4} (#3) ;
}

\newcommand{\colorweigedge}[7][]{
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [-,line width=0.6pt,#1] (\y) ;
      % \draw[rounded corners] ($(\x)!0.5!(\y)$) rectangle node{#4} (\y) ;
      \pgfmathparse{width("\noexpand\noexpand\noexpand#4")} ; %the width calc
      \pgfmathsetlength{\mywidth}{\pgfmathresult} ; % Put it into a length register
      \pgfmathparse{height("\noexpand\noexpand\noexpand#4")} ; %the height calc
      \pgfmathsetlength{\myheight}{\pgfmathresult} ; % Put it into a length register
      \node[rectangle,draw,rounded corners=0.4\myheight,line width=0.6pt,color=#5,fill=#6,text=#7,minimum height=1.8\myheight,minimum width=1.2\mywidth,label={center:\textcolor{#7}{#4}}] at ($(\x)!0.5!(\y)$) {} ;
    } ;
  } ;
}

\newcommand{\ellipsis}[2]{
  \node at ($(#1)!.5!(#2)$) {\ldots} ;
}

\newcommand{\annotatenode}[4]{
  \node[] at ([xshift=#3,yshift=#4]#1) {#2} ;
}

\newcommand{\colorfulannotnode}[6]{
  \pgfmathparse{width("\noexpand\noexpand\noexpand#2")} ; %the width calc
  \pgfmathsetlength{\mywidth}{\pgfmathresult} ; % Put it into a length register
  \pgfmathparse{height("\noexpand\noexpand\noexpand#4")} ; %the height calc
  \pgfmathsetlength{\myheight}{\pgfmathresult} ;
  \node[rectangle,draw,rounded corners=0.4\myheight,line width=0.6pt,color=#5,fill=#5,text=#6,minimum height=1.3\myheight,minimum width=1.3\mywidth,label={center:\textcolor{#6}{#2}}] at ([xshift=#3,yshift=#4]#1) {} ;
}

\newcommand{\midlinewidth}{1.0pt}
\newcommand{\incmidlinewidth}{1.7pt}
\newcommand{\largelinewidth}{1.9pt}
\newcommand{\xlargelinewidth}{2.3pt}
\newcommand{\middist}{17pt}
\newcommand{\sqintermiddist}{15.5pt}
\newcommand{\intermiddist}{30pt}
\newcommand{\largedist}{49pt}
\newcommand{\midsmalldist}{10pt}
\newcommand{\smalldist}{6pt}
\newcommand{\tinydist}{4pt}
\newcommand{\centraldist}{30pt}
\newcommand{\midlargedist}{24pt}
\newcommand{\halfdist}{19pt}
\newcommand{\weightsize}{\fontsize{10}{10}\selectfont}
\newcommand{\annotsize}{\fontsize{10}{10}\selectfont}

\definecolor{lacamlilac} {RGB} {107,93,153}
\definecolor{lacamlilac2} {RGB} {93, 109, 152}
\definecolor{lacamlightlilac} {RGB} {174, 166, 201}
\definecolor{lacamdarklilac} {RGB} {51, 10, 102}
\definecolor{lacamdarklilac5} {RGB} {51, 10, 102}
\colorlet{lacamdarklilac4} {lacamdarklilac5!80!}
\colorlet{lacamdarklilac3} {lacamdarklilac5!60!}
\colorlet{lacamdarklilac2} {lacamdarklilac5!40!}
\colorlet{lacamdarklilac1} {lacamdarklilac5!20!}

\definecolor{lacamgold5} {RGB} {255, 87, 0}
\colorlet{lacamgold4} {lacamgold5!80!}
\colorlet{lacamgold3} {lacamgold5!60!}
\colorlet{lacamgold2} {lacamgold5!40!}
\colorlet{lacamgold1} {lacamgold5!20!}
\definecolor{violet} {RGB} {119, 111, 178}
\definecolor{petroil2} {RGB} {36, 165, 175}
\definecolor{petroil4} {RGB} {30, 132, 149}
\definecolor{petroil6} {RGB} {23, 101, 115}
\definecolor{gold2} {RGB} {255, 130, 0}
\definecolor{gold4} {RGB} {250, 100, 0}
\definecolor{gold6} {RGB} {245, 90, 0}

\definecolor{lacamoil5}{rgb}{0.13, 0.67, 0.8}
\colorlet{lacamoil4} {lacamoil5!80!}
\colorlet{lacamoil3} {lacamoil5!60!}
\colorlet{lacamoil2} {lacamoil5!40!}
\colorlet{lacamoil1} {lacamoil5!20!}

\definecolor{lightgray} {RGB} {210, 210, 210}
\definecolor{myblue} {RGB} {80, 145, 207}
\definecolor{mypurple} {RGB} {101, 43, 150}
\definecolor{myred} {RGB} {255, 0, 1}

%\definecolor{tomato0} {HTML} {E57373}
\definecolor{tomato0} {HTML} {EF9A9A}
\definecolor{tomato1} {HTML} {F44336}
\definecolor{tomato2} {HTML} {E53935}
\definecolor{tomato3} {HTML} {D32F2F}
\definecolor{tomato4} {HTML} {C62828}
\definecolor{tomato5} {HTML} {B71C1C}


\definecolor{peas1} {HTML} {009688}
\definecolor{peas2} {HTML} {00897B}
\definecolor{peas3} {HTML} {00796B}
\definecolor{peas4} {HTML} {00695C}
\definecolor{peas5} {HTML} {004D40}

\definecolor{bgrey0} {HTML} {78909C}
\definecolor{bgrey1} {HTML} {607D8B}
\definecolor{bgrey2} {HTML} {546E7A}
\definecolor{bgrey3} {HTML} {455A64}
\definecolor{bgrey4} {HTML} {37474F}
\definecolor{bgrey5} {HTML} {263238}

\definecolor{olive0} {HTML} {C5E1A5}
\definecolor{olive1} {HTML} {AED581}
\definecolor{olive2} {HTML} {9CCC65}
\definecolor{olive3} {HTML} {8BC34A}
\definecolor{olive4} {HTML} {7CB342}
\definecolor{olive5} {HTML} {689F38}

\definecolor{pink0} {HTML} {FCE4EC}
\definecolor{pink1} {HTML} {F8BBD0}
\definecolor{pink2} {HTML} {F48FB1}
\definecolor{pink3} {HTML} {F06292}
\definecolor{pink4} {HTML} {EC407A}
\definecolor{pink5} {HTML} {FF80AB}

\definecolor{brown0} {HTML} {D7CCC8}
\definecolor{brown1} {HTML} {BCAAA4}
\definecolor{brown2} {HTML} {A1887F}
\definecolor{brown3} {HTML} {8D6E63}
\definecolor{brown4} {HTML} {795548}
\definecolor{brown5} {HTML} {6D4C41}
\definecolor{brown6} {HTML} {5D4037}

\definecolor{yellow0} {HTML} {CDDC39}
\definecolor{yellow1} {HTML} {9E9D24}
\definecolor{yellow3} {HTML} {FFBD2A}
\definecolor{yellow4} {HTML} {FFB000}
\definecolor{yellow5} {HTML} {FFD600}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:
